How to Make Traversable Wormholes: Eternal AdS$_4$ Wormholes from Coupled CFT's

We construct an eternal traversable wormhole connecting two asymptotically $\text{AdS}_4$ regions. The wormhole is dual to the ground state of a system of two identical holographic CFT's coupled via a single low-dimension operator. The coupling between the two CFT's leads to negative null energy in the bulk, which supports a static traversable wormhole. As the ground state of a simple Hamiltonian, it may be possible to make these wormholes in the lab or on a quantum computer.

==> MMP.tex <==

\section{MMP Wormhole}
\label{S:MMP}

In this section we will review the wormhole construction of MMP. MMP find a long traversable wormhole embedded in four dimensional Minkowski space by considering two near extremal Reissner Nordstr\"{o}m black holes. The wormhole crucially depends on a Casimir-like energy that is created by fermions traveling along electromagnetic field lines between the black holes. The negative energy produced by the fermions then gives rise to a wormhole geometry that connects the black holes through an $\text{AdS}_2\times S^2$ like throat. The wormhole geometry consists of three regions in which the metric can be approximated, namely the the wormhole, the mouth and the flat space region. The solution in each of the three limits has an overlapping region of validity in which the metrics can be patched together by matching conditions. 

The magnetically charged black hole permits a magnetic field field on the sphere. Massless charged fermions (with charge one) moving along the field lines give rise to a series of Landau levels. Crucially for massless charged fermions the energy of the lowest Landau vanishes, so that we have zero energy modes on the sphere. Each of these modes correspond to a massless two dimensional field in the time and radial direction. Effectively we thus have two dimensional massless fermions traveling along the magnetic field lines. They travel between the black holes (of opposite magnetic charge $q$, which is assumed to be large) into their mouths, and through the wormhole, so that they move in a circle. If this circle has length $L$, the total energy of the configuration equals
\begin{equation}
E=\frac{q}{24}\frac{\pi}{L}-\frac{q}{12}\frac{2\pi}{L}=-\frac{q\pi}{8L},
\end{equation} 
where the first contribution comes from the conformal anomaly, while the second term is the Casimir-like contribution. With this negative energy the Einstein equations are solved in the wormhole region, and the resulting geometry is a perturbation of $\text{AdS}_2\times S^2$ in global coordinates. This geometry can be matched to the near horizon limit of the black hole geometry by the following matching condition
\begin{equation}
2\frac{r-r_e}{r_e}\sim\frac{\pi\alpha}{2}\rho.
\end{equation}
Here $r$ is the radial coordinate in the black hole geometry, $r_e$ is the radius of the horizon of the extremal RN black hole, $\rho$ is the radial coordinate of the global AdS metric in the wormhole, and $\alpha$ is a constant. 

The resulting wormhole can be stabilised by considering the wormhole mouths to be rotating around one another to counteract the attracting electromagnetic force between the oppositely charged black holes. However this rotation is slow enough to ascertain that the massless charged fermions and the negative energy they create are protected from effects of this rotation. Thus resulting in a wormhole that has no horizons and is stable for a finite amount of time.

